DAVE: Distribution-aware Attribution via ViT Gradient Decomposition

Vision Transformers (ViTs) have become a dominant architecture in computer vision, yet producing stable and high-resolution attribution maps for these models remains challenging. Architectural components such as patch embeddings and attention routing often introduce structured artifacts in pixel-level explanations, causing many existing methods to rely on coarse patch-level attributions. We introduce DAVE \textit{(\underline{D}istribution-aware \underline{A}ttribution via \underline{V}iT Gradient D\underline{E}composition)}, a mathematically grounded attribution method for ViTs based on a structured decomposition of the input gradient. By exploiting architectural properties of ViTs, DAVE isolates locally equivariant and stable components of the effective input--output mapping. It separates these from architecture-induced artifacts and other sources of instability.

==> figures/1-1_teaser.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{images/panoramic_3.pdf}
    \caption{\textbf{DAVE attributions for DeiT III-B-16/224.} ImageNet-1k samples (left) and corresponding pixel-level DAVE attributions (right).}
    \label{fig:teaser}
\end{figure}

==> figures/class_consistency.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.95\linewidth]{images/consistency.pdf}
    \caption{\textbf{Class-consistent attributions.} DAVE consistently highlights similar visual features associated with the model’s prediction for \textit{giant panda}, such as the eyes and ears. (DeiT-III-B-16 model)}
    \vspace{-2mm}
    \label{fig:class_consistency}
\end{figure}

==> figures/dave_qual_comparison_deit3_5.tex <==
% --- GridPG figure ---
\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{images/qual_final_deit3_base_stripped_5.pdf}
\caption{\textbf{Qualitative comparison of attribution maps.} For a set of ImageNet examples (rows), we show the input image (left) and attribution maps produced by C-LRP, LeGrad, AttnLRP, Integrated Gradients, SmoothGrad, and Dave (ours) (columns). Dave yields sharper, more object-aligned explanations with reduced background noise compared to prior methods.
\adam{J: maybe full width? / eqrlier?}
}

  \label{fig:dave_vs_rest_deit3_base_5}
\end{figure*}

==> figures/dave_qual_comparison_deit3_8.tex <==
% --- GridPG figure ---
\begin{figure}[!t]
  \centering
  \includegraphics[width=\columnwidth]{images/qual_final_deit3_base_stripped_8.pdf}
\caption{\textbf{Qualitative comparison of attribution maps.} For a set of ImageNet examples (rows), we show the input image (left) and attribution maps produced by C-LRP, LeGrad, AttnLRP, Integrated Gradients, SmoothGrad, and Dave (ours) (columns). Dave yields sharper, more object-aligned explanations with reduced background noise compared to prior methods.
\adam{J: maybe full width? / eqrlier?}
}

  \label{fig:dave_vs_rest_deit3_base_8}
\end{figure}

==> figures/epg_eval.tex <==
% --- EPG figure ---
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{images/epg_std_bcos.png}
  \caption{EPG localization (\%) across ViT-B/16-based model variants. Each curve corresponds to an attribution method; DAVE (ours) is highlighted in blue.}
  \label{fig:epg}
\end{figure}

==> figures/gridpg_eval.tex <==

% --- GridPG figure ---
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{images/gridpg_eval.png}
  \caption{GridPG localization (\%) across ViT-B/16-based model variants. Each curve corresponds to an attribution method; DAVE (ours) is highlighted in blue.}
  \label{fig:gridpg}
\end{figure}

==> figures/pixel_del.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{images/deit3_pixel_del.png}
  \caption{Pixel Deletion (\%) across DeitIII-B/16-based model across attribution methods. Each curve corresponds to an attribution method; DAVE (ours) is highlighted in purple. \sid{TODO: update, make prettier}}
  \label{fig:deit3_pixel_del}
\end{figure}

==> sections/method.tex <==
% \section{Old Method}
% DAVE defines attribution as the expected direct contribution over a local input distribution. The method consists of two steps. First, we express a Vision Transformer as dynamic linear operator, which yields a local attribution probe corresponding to the direct input contribution (Section~\ref{sec:exact_decomposition}).
% Second, we define the attribution as an expectation of this probe over a neighborhood inputs, which additionally suppresses structural artifacts induced by patch tokenization, positional encoding, and discrete attention routing (Section~\ref{sec:distribution_aware}).
% Together, these steps produce stable, neighborhood-aware, and class-consistent attributions.

% \subsection{ViT decomposition}\label{sec:exact_decomposition}
% We interpret the Vision Transformer (ViT) as a composition of dynamic linear operators with additional bias parameters. This allows to extract effective weight of a direct contribution, applied to model's input, as a single attribution probe.

% \paragraph{Why not Jacobian.}

% \paragraph{Layer structure.}
% We model each Vision Transformer (ViT) layer as a dynamic linear operator
% followed by a constant addition. Let $F_i : V^{(i-1)}_{in} \times V^{(i-1)}_{cond} \to V^{(i)}_{in}$ denote the layer map:
% \begin{equation}\label{eq:vit_layer}
% F_i(\boldsymbol{X}, \boldsymbol{Z})
% \;:=\;
% L_i(\boldsymbol{Z})(\boldsymbol{X})
% \;+\;
% \boldsymbol{B}_i
% \end{equation}
% where $L_i(\boldsymbol{Z}) \in \mathcal{L}(V_{in}^{(i-1)}, V_{in}^{(i)})$
% is a conditioned linear operator acting on input $\boldsymbol{X}$,
% and $\boldsymbol{B}_i \in V_{in}^{(i)}$ is a static bias term.


% \paragraph{Layer representation.}
% Motivated by the architectural structure of ViT layers, we identify layer inputs and
% outputs with matrices in $\mathbb{R}^{t \times d_{i-1}}$ and $\mathbb{R}^{t \times d_i}$,
% respectively, where $t$ denotes the number of tokens and $d_i$ the token dimensionality.
% Under this identification, we consider two classes of dynamic linear operators
% $L_i$:
% \begin{equation}\label{eq:layer_representation}
% \begin{split}
% (\text{I})& \quad
% L_i(\boldsymbol{Z})(\boldsymbol{X})
% := \boldsymbol{W}_t(\boldsymbol{Z})\,\boldsymbol{X}\,\boldsymbol{W}_d\\
% (\text{II})& \quad
% L_i(\boldsymbol{Z})(\boldsymbol{X})
% := \boldsymbol{\Phi}(\boldsymbol{Z}) \odot \boldsymbol{X}
% \end{split}
% \end{equation}
% where $\boldsymbol{W}_t(\boldsymbol{Z}) \in \mathbb{R}^{t \times t}$ is a
% condition-dependent token-mixing matrix,
% $\boldsymbol{W}_d \in \mathbb{R}^{d_{i-1} \times d_i}$ is a static dimensional projection,
% and $\boldsymbol{\Phi}(\boldsymbol{Z}) \in \mathbb{R}^{t \times d_{i-1}}$ is a
% condition-dependent gating matrix.
% For fixed conditioning variable $\boldsymbol{Z}$, both constructions are linear in
% $\boldsymbol{X}$.

% These operators cover all major ViT components, including attention, normalization, and pointwise activations; details are provided in the Appendix.

% \paragraph{Diagonal evaluation.}
% Each layer map
% $F_i : V^{(i-1)}_{in} \times V^{(i-1)}_{cond} \to V^{(i)}_{in}$
% is defined on separate input and conditioning variables.
% In Vision Transformers, layers are evaluated on the \emph{diagonal}, meaning that the
% conditioning variable takes the same numerical value as the input at evaluation time.
% Formally, we evaluate $F_i(\boldsymbol{X}, \boldsymbol{Z})$ at points where
% $\boldsymbol{Z}$ and $\boldsymbol{X}$ have identical coordinate representations $[\boldsymbol{Z}]_{\mathcal{B}_{cond}} = [\boldsymbol{X}]_{\mathcal{B}_{in}}$, while
% still treating them as distinct arguments of the function. This allows to separate the direct and indirect contributions of the layer (see Equation~\ref{eq:contributions}), which are otherwise entangled in the model's Jacobian.


% \paragraph{ViT representation.}
% A network with $n$ layers defines a map
% $\mathcal{F} :
% V^{(0)}_{in}
% \times
% \prod_{i=0}^{n-1} V^{(i)}_{cond}
% \;\longrightarrow\;
% V^{(n)}_{in}$ specified recursively by:
% \[
% \boldsymbol{X}_0 = \boldsymbol{X}, \qquad
% \boldsymbol{X}_{i+1} = F_i(\boldsymbol{X}_i, \boldsymbol{Z}_i),
% \]
% where $\boldsymbol{X}$ denotes the network input and
% $\boldsymbol{Z} := (\boldsymbol{Z}_0,\ldots,\boldsymbol{Z}_{n-1})$
% collects all conditioning variables.
% The network output is
% $\boldsymbol{X}_n = \mathcal{F}(\boldsymbol{X}, \boldsymbol{Z})$.

% Under diagonal evaluation, each conditioning variable $\boldsymbol{Z}_i$ is chosen to
% have the same numerical value as the corresponding layer input $\boldsymbol{X}_i$,
% so the forward pass is fully determined by $\boldsymbol{X}$.




% \paragraph{ViT decomposition.}
% Since each layer $F_i$ is affine in its input, the network map $\mathcal{F}$ admits the
% decomposition
% \begin{equation}
% \mathcal{F}(\boldsymbol{X}, \boldsymbol{Z})
% =
% L_{\mathcal{F}}(\boldsymbol{Z})(\boldsymbol{X})
% +
% \sum_{i=1}^{n}
% L_{\mathcal{F}_i}(\boldsymbol{Z})(\boldsymbol{B}_i),
% \end{equation}
% where $L_{\mathcal{F}}(\boldsymbol{Z})
% = \prod_{i=1}^{n} L_i(\boldsymbol{Z}_i)$
% denotes the effective dynamic linear operator obtained by composing all dynamic linear layers.
% Following Eq.~\ref{eq:contributions}, the direct contribution
% $L_{\mathcal{F}}(\boldsymbol{Z})$ is given by the partial derivative
% $D_{\boldsymbol{X}}\mathcal{F}(\boldsymbol{X}, \boldsymbol{Z})$.


% Note that this direct contribution is not the standard Jacobian of the ViT and does not represent input sensitivity of the original model. Since input and conditioning variables are treated separately, it disentangles the transformation that the model applies directly to the input (direct input contribution), from the conditioning of this transformation (indirect contribution).



% \paragraph{Attribution probe.}
% As the direct contribution $L_{\mathcal{F}}(\boldsymbol{Z})$ summarizes the transformation that the ViT applies directly to the input $\boldsymbol{X}$, we use its effective weight $\boldsymbol{W}_{\mathcal{F}}(\boldsymbol{Z})$ 
% as an attribution probe (see Equation~\ref{eq:effective_weight}), assuming a scalar-valued output
% $V_{\mathrm{out}}=\mathbb{R}$. 

% In DAVE, this probe is treated as a local estimator and averaged over a neighborhood of inputs, thereby aggregating direct contributions across a family of nearby frozen attention, normalization, and activation states.


% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/evolution.pdf}
%     \caption{Progressive construction of the DAVE attribution for images from the same class (red panda).
%     Columns show: standard input $\times$ gradient, attribution probe $\boldsymbol{W}_F(\boldsymbol{X})\odot\boldsymbol{X}$, locally equivariant contribution $\boldsymbol{W}^{\star}_F(\boldsymbol{X})\odot\boldsymbol{X}$, and the final DAVE attribution after low-pass
%     filtering in the contribution domain. DAVE reveals consistent,
%     class-specific features across images.}
%     \label{fig:evolution}
% \end{figure}

% \subsection{Distribution-aware}\label{sec:distribution_aware}
% The effective weight of direct contribution provides a pointwise summary of the
% transformation applied directly to the input. However, it ignores the indirect conditioning contribution and 
% also contains components that arise from architectural constraints (e.g.,
% non-overlapping patch embeddings) or local high-frequency
% patterns in the contribution space. In this section, we introduce distribution-aware
% neighborhood averaging designed suppress such artifacts by promoting local
% consistency of direct contributions.

% \subsubsection{Local equivariance}

% Vision models trained with data augmentation are often stable under small, invertible spatial transformations
% $\tau : V_{\mathrm{in}} \rightarrow V_{\mathrm{in}}$, such that
% $F(\tau(\boldsymbol{X})) \approx F(\boldsymbol{X})$.
% Under this assumption, we seek attribution signals that are approximately equivariant to such transformations, 
% treating strongly non-equivariant components as likely artifacts. In other words, we look for:
% \begin{equation}\label{eq:equivariance}
% \boldsymbol{W}^{\star}_F(\boldsymbol{X})
% \approx
% [\tau^{-1}\!\circ\boldsymbol{W}_F\circ\tau](\boldsymbol{X})
% \end{equation}

% To suppress components of $\boldsymbol{W}_F(\boldsymbol{X})$ that violate this
% local consistency, we apply a Reynolds-style averaging operator over a
% neighborhood of small transformations. Let $G$ be a compact group of spatial
% transformations (e.g., rotations), and let $\nu$ be a probability measure
% supported in a neighborhood of the identity. We define:
% \begin{equation}
% \boldsymbol{W}^{\star}_F(\boldsymbol{X})
% =
% \int_G
% [\tau^{-1}\circ\boldsymbol{W}_F\circ\tau](\boldsymbol{X})
% \, d\nu(\tau).
% \end{equation}

% This averaging preserves components of $\boldsymbol{W}_F(\boldsymbol{X})$ that
% are stable under transformations in $G$, while attenuating non-equivariant
% artifacts (see Figure~\ref{fig:evolution}, columns~3 and~4). In the limit where
% $\nu$ approaches the uniform Haar measure, the operator reduces to the classical
% Reynolds projection onto the space of $G$-invariant attributions.

\subsubsection{Low-pass filtering}
Finally, to suppress high-frequency artifacts in the contribution domain, we  apply
a smoothing operation inspired by classical signal processing. Specifically, we
perform Gaussian perturbations in the input space and average the resulting
contributions, which is equivalent to convolving the contribution map with a
Gaussian kernel (see Appendix for derivation):
\begin{equation}
\tilde{\boldsymbol{W}}^{eq}_L(\boldsymbol{x})
=
\mathbb{E}_{\boldsymbol{\epsilon} \sim \mathcal{N}(0,\Sigma)}
\left[
\boldsymbol{W}^{eq}_L(\boldsymbol{x} + \boldsymbol{\epsilon})
\right]
=
(\boldsymbol{W}^{eq}_L \ast \mathcal{K})(\boldsymbol{x})
\end{equation}
where $\mathcal{K}$ denotes the corresponding Gaussian kernel. This operation
acts as a low-pass filter, attenuating high-frequency components that are unlikely
to be stable under small input perturbations.


\subsection{DAVE framework}
Combining transformation averaging and Gaussian smoothing, the final
distribution-aware effective weight is obtained by taking the expectation of
the effective weight under local input perturbations:
\[
\tilde{\boldsymbol{W}}^{eq}_L(\boldsymbol{X})
=
\mathbb{E}_{\tau \sim \nu,\;\boldsymbol{\epsilon} \sim \mathcal{N}(0,\Sigma)}
\left[
\tau^{-1}\!\left(
\boldsymbol{W}_L(\tau(\boldsymbol{X}) + \boldsymbol{\epsilon})
\right)
\right]
\]
where $\tau \sim \nu$ is a random spatial transformation drawn from a probability
measure supported in a neighborhood of the identity, and
$\boldsymbol{\epsilon} \sim \mathcal{N}(0,\Sigma)$ denotes additive Gaussian
noise.

The final DAVE attribution is then defined by applying the
distribution-aware effective weight to the input via element-wise
multiplication:
\begin{equation}
\mathrm{DAVE}(L,\boldsymbol{X})
=
\tilde{\boldsymbol{W}}^{eq}_F(\boldsymbol{X}) \odot \boldsymbol{X}
\end{equation}



% \begin{algorithm}[t]
% \caption{DAVE: Distribution-Aware Direct Attribution for ViTs}
% \label{alg:dave}
% \begin{algorithmic}[1]
% \REQUIRE Input $\mathbf{x}$, model $F$, transformation group $G$, local measure $\nu$ on $G$, noise std.\ $\sigma$, number of samples $K$

% \STATE $\mathbf{w} \leftarrow \mathbf{0}$ \COMMENT{accumulator for effective weights}

% \FOR{each step $k$}
%     \STATE $\tau \sim \nu$,  $\boldsymbol{\epsilon} \sim \mathcal{N}(\mathbf{0}, \sigma^{2}\mathbf{I})$
%     \STATE $\mathbf{x}_k \leftarrow \tau(\mathbf{x} + \boldsymbol{\epsilon})$
%     \STATE $\mathbf{x}_i \leftarrow \mathbf{x}_k$
    
%     \FOR{each layer $i$}
%         \STATE $\mathbf{z}_i \leftarrow \mathrm{detach}(\mathbf{x}_i)$ \COMMENT{conditioning variable}
%         \STATE $\mathbf{x}_i \leftarrow F_i(\mathbf{x}_i,\mathbf{z}_i)$
%     \ENDFOR
    
%     \STATE $\mathbf{w}_k \leftarrow \nabla^{(detached)}_{\mathbf{x}_k}x_i$ \COMMENT{effective weight}
%     \STATE $\mathbf{w} \leftarrow \mathbf{w} + \tau^{-1}(\mathbf{w}_k)$ 
% \ENDFOR

% \STATE $\mathbf{w} \leftarrow \mathbf{w} / K$
% \STATE \textbf{return} $\mathbf{x} \odot \mathbf{w}$
% \end{algorithmic}
% \end{algorithm}









% %\paragraph{Layer examples.}
% % Type I layers include: Fully-connected, where $\boldsymbol{W}_t(\boldsymbol{Z}) = \boldsymbol{I}_{t}$; Self-attention, where $\boldsymbol{W}_t(\boldsymbol{Z})$ represents softmaxed attention scores, and $\boldsymbol{W}_d$ represents output mapping with potential bias $\boldsymbol{B}$; Layer normalization, where $\boldsymbol{W}_d = \boldsymbol{I}_d - \frac{1}{d}\mathbf{1}\mathbf{1}^\top$ is a centering matrix, $\boldsymbol{W}_t(\boldsymbol{Z})[i, i] = \gamma/\sigma(\boldsymbol{Z}[i, :])$ is a diagonal, per-token, standard deviation scaling matrix, and $\boldsymbol{B}$ represents a static offset (see Appendix for derivations).

% % Type II layers include: element-wise nonlinear activation functions such as GELU, where $\boldsymbol{\Phi(\boldsymbol{Z})}$ is the Cumulative Distribution Function for Gaussian Distribution; SWISH, where $\boldsymbol{\Phi}(\boldsymbol{Z}) = \text{sigmoid}(\boldsymbol{Z})$.

==> sections/preliminaries.tex <==
% \section{Old stuff}
% Why dynamic linear?

% \subsection{Dynamic Linear Operators}\label{sec:dynamic_linear}
% Dynamic linear operators are linear transformations conditioned nonlinearly on a conditioning variable. This makes them nonlinear with respect to this variable but linear with respect to the input, enabling a principled separation between direct linear input contributions and indirect effects arising from the conditioning dependence of the transformation.

% \paragraph{Definition.}
% Let $V_{\mathrm{in}}$, $V_{\mathrm{cond}}$, $V_{\mathrm{out}}$ be finite-dimensional real vector spaces.
% A \emph{dynamic linear operator} is a differentiable map
% $L : V_{\mathrm{cond}} \to \mathcal{L}(V_{\mathrm{in}}, V_{\mathrm{out}})$ that induces an associated map $F : V_{\mathrm{in}} \times V_{\mathrm{cond}} \to V_{\mathrm{out}}$:

% \begin{equation}\label{eq:application}
% F(\boldsymbol{X},\boldsymbol{Z}) := L{(\boldsymbol{Z})}(\boldsymbol{X})
% \end{equation}

% \paragraph{Linearity.} Due to linearity of $L(\boldsymbol{Z})$, $F$ is linear in the input $\boldsymbol{X}$ when conditioning variable $\boldsymbol{Z}$ is held constant. Consequently, it inherits the algebraic properties of linear maps with respect to the input $\boldsymbol{X}$, including distributivity over addition, closure under residual connections, and closure under composition with other dynamic linear layers with fixed conditioning variables (see Appendix for derivations).

% \paragraph{Direct and Indirect Contributions.}
% For fixed conditioning variable, the dependence on the input \( \boldsymbol{X} \) is linear and fully determined by the effective operator \( L(\boldsymbol{Z}) \), constituting the \emph{direct contribution} of the input. In contrast, the \emph{indirect contribution} of the conditioning variable arises through its influence on the operator itself. Infinitesimally, this distinction is captured by the partial derivatives:
% \begin{equation}\label{eq:contributions}
% \begin{split}
%  D_{\boldsymbol{X}} F(\boldsymbol{X}, \boldsymbol{Z}) &= L(\boldsymbol{Z}) \\ D_{\boldsymbol{Z}} F(\boldsymbol{X},\boldsymbol{Z}) &= (D L(\boldsymbol{Z}))[\boldsymbol{X}]
% \end{split}
% \end{equation}


% \paragraph{Effective Weight.} For a specific bases $\mathcal{B}_{in}$ of $V_{in}$ and  $\mathcal{B}_{out}$ of $V_{out}$, the linear map $L{(\boldsymbol{Z})}$ admits a matrix
% representation of an \emph{effective weight} $\boldsymbol{W}_F(\boldsymbol{Z}) \in \mathbb{R}^{d_{\mathrm{out}} \times d_{\mathrm{in}}}$,
% and the function can be written as:
% \begin{equation}\label{eq:effective_weight}
%     [F(\boldsymbol{X}, \boldsymbol{Z})]_{\mathcal{B}_{out}} = \boldsymbol{W}_F(\boldsymbol{Z})[\boldsymbol{X}]_{\mathcal{B}_{in}}
% \end{equation}

% In this coordinate representation, the entry
% $\boldsymbol{W}_F(\boldsymbol{Z})[j,i]\boldsymbol{X}_{\mathcal{B}_{\mathrm{in}}}[i]$
% quantifies the additive contribution of the $i$-th input coordinate to the $j$-th output coordinate, which makes it a suitable attribution for dynamic linear operators.

==> tables/epg_localisation.tex <==
% \begin{table}[t]
%   \centering
%   \caption{EPG localisation scores on ImageNet, comparing state-of-the-art explanation methods against DAVE (ours) for ViT-B/16-based architectures.}
%   \label{tab:gridpg}

%   \scriptsize
%   \setlength{\tabcolsep}{3pt}         % tighter columns
%   \renewcommand{\arraystretch}{0.95}  % tighter rows

%   \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{5}{c}{\textbf{EPG} $\uparrow$} \\
%     \cmidrule(lr){2-6}
%      & \textbf{IxG} & \makecell{\textbf{Chefer-}\\\textbf{CAM}} & \textbf{LeGrad} & \textbf{B-cos} & \textbf{DAVE} \\
%     \midrule
%     ViT-B/16         & -- & -- & -- & -- & -- \\
%     DeiT-B/16        & -- & -- & -- & -- & -- \\
%     Bcos-ViT-B/16    & -- & -- & -- & -- & -- \\
%     Bcos-ViT\_c-B/16 & -- & -- & -- & -- & -- \\
%     DINO-ViT-B/16    & -- & -- & -- & -- & -- \\
%     CLIP-ViT-B/16    & -- & -- & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}[t]
%   \centering
%   \caption{EPG localisation scores on ImageNet, computed on $2{\times}2$ grids with cell size $224{\times}224$, comparing state-of-the-art explanation methods against DAVE (ours) for ViT-B/16-based architectures. Scores are reported as mean$\pm$std (over $n{=}10k$ images).}
%   \label{tab:epg}

%   \scriptsize
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{0.92}

%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{6}{c}{\textbf{EPG} $\uparrow$} \\
%     \cmidrule(lr){2-7}
%     & \textbf{IxG}
%     & \makecell{\textbf{Attn}\\\textbf{LRP}}
%     & \textbf{IG}
%     & \makecell{\textbf{C-}\\\textbf{CAM}}
%     & \textbf{B-cos}
%     & \textbf{DAVE} \\
%     \midrule
%     ViT-B/16
%       & $\mstd{0.57}{0.34}$
%       & $\mstd{0.62}{0.32}$
%       & $\mstd{0.55}{0.33}$
%       & $\mstd{0.72}{0.23}$
%       & --
%       & $\textcolor{blue}{\mathbf{\mstd{0.79}{0.27}}}$ \\
%     DeiT-B/16
%       & $\mstd{0.61}{0.29}$
%       & $\mstd{0.59}{0.30}$
%       & $\mstd{0.60}{0.29}$
%       & $\mstd{0.68}{0.27}$
%       & --
%       & $\textcolor{blue}{\mathbf{\mstd{0.77}{0.26}}}$ \\
%     Bcos-ViT-B/16
%       & $\mstd{0.64}{0.29}$
%       & --
%       & $\mstd{0.61}{0.29}$
%       & --
%       & $\mstd{0.75}{0.25}$
%       & $\mstd{0.70}{0.30}$ \\
%     Bcos-ViT\_c-B/16
%       & $\mstd{0.65}{0.28}$
%       & --
%       & $\mstd{0.64}{0.28}$
%       & --
%       & $\mstd{0.69}{0.28}$
%       & $\textcolor{blue}{\mathbf{\mstd{0.73}{0.30}}}$ \\
%     DeiT-III/16
%       & $\mstd{0.59}{0.31}$
%       & $\mstd{0.64}{0.29}$
%       & $\mstd{0.56}{0.31}$
%       & --
%       & --
%       & $\textcolor{blue}{\mathbf{\mstd{0.76}{0.28}}}$ \\
%     CLIP-ViT-B/16 & -- & -- & -- & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}%
%   }
% \end{table}



\begin{table}[t]
  \centering
  \caption{EPG localisation scores on ImageNet, comparing attribution methods across ViT-B/16-based architectures. Scores are reported as mean$\pm$std (over $n{=}10k$ images) and shown as percentages.}
  \label{tab:epg_transposed_pct}

  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{0.92}

  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lccccc}
    \toprule
    \textbf{Method} & \textbf{ViT-B/16} & \textbf{DeiT-B/16} & \textbf{DeiT-III/16} & \textbf{Bcos-ViT-B/16} & \textbf{Bcos-ViT\_c-B/16} \\
    \midrule
    IxG
      & $\mstd{57}{34}\%$
      & $\mstd{61}{29}\%$
      & $\mstd{59}{31}\%$
      & $\mstd{64}{29}\%$
      & $\mstd{65}{28}\%$ \\
    AttnLRP
      & $\mstd{62}{32}\%$
      & $\mstd{59}{30}\%$
      & $\mstd{64}{29}\%$
      & --
      & -- \\
    IG
      & $\mstd{55}{33}\%$
      & $\mstd{60}{29}\%$
      & $\mstd{56}{31}\%$
      & $\mstd{61}{29}\%$
      & $\mstd{64}{28}\%$ \\
    C-CAM
      & $\mstd{72}{23}\%$
      & $\mstd{68}{27}\%$
      & --
      & --
      & -- \\
    B-cos
      & --
      & --
      & --
      & $\mstd{75}{25}\%$
      & $\mstd{69}{28}\%$ \\
    DAVE
      & $\textcolor{blue}{\mathbf{\mstd{79}{27}}}\%$
      & $\textcolor{blue}{\mathbf{\mstd{77}{26}}}\%$
      & $\textcolor{blue}{\mathbf{\mstd{76}{28}}}\%$
      & $\mstd{70}{30}\%$
      & $\textcolor{blue}{\mathbf{\mstd{73}{30}}}\%$ \\
    \bottomrule
  \end{tabular}%
  }
\end{table}

==> tables/gridpg_localisation.tex <==
% \begin{table}[t]
%   \centering
%   \caption{GridPG localisation scores on ImageNet, computed on $2{\times}2$ grids with cell size $224{\times}224$, comparing state-of-the-art explanation methods against DAVE (ours) for ViT-B/16-based architectures.}
%   \label{tab:gridpg}

%   \scriptsize
%   \setlength{\tabcolsep}{3pt}         % tighter columns
%   \renewcommand{\arraystretch}{0.95}  % tighter rows

%   \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{5}{c}{\textbf{GridPG} $\uparrow$} \\
%     \cmidrule(lr){2-6}
%      & \textbf{IxG} & \makecell{\textbf{Chefer-}\\\textbf{CAM}} & \textbf{LeGrad} & \textbf{B-cos} & \textbf{DAVE} \\
%     \midrule
%     ViT-B/16         & -- & -- & -- & -- & -- \\
%     DeiT-B/16        & -- & -- & -- & -- & -- \\
%     Bcos-ViT-B/16    & -- & -- & -- & -- & -- \\
%     Bcos-ViT\_c-B/16 & -- & -- & -- & -- & -- \\
%     DINO-ViT-B/16    & -- & -- & -- & -- & -- \\
%     CLIP-ViT-B/16    & -- & -- & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% preamble:
% \usepackage{xcolor}

% \begin{table}[t]
%   \centering
%   \caption{GridPG localisation scores on ImageNet, computed on $2{\times}2$ grids with cell size $224{\times}224$, comparing state-of-the-art explanation methods against DAVE (ours) for ViT-B/16-based architectures. Scores are reported as mean$\pm$std (over $n{=}32$ images).}
%   \label{tab:gridpg}

%   \scriptsize
%   \setlength{\tabcolsep}{3pt}
%   \renewcommand{\arraystretch}{0.95}

%   \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{5}{c}{\textbf{GridPG} $\uparrow$} \\
%     \cmidrule(lr){2-7}
%      & \textbf{IxG} & \textbf{AttnLRP} & \textbf{IG} & \textbf{C-CAM} & \textbf{B-cos} & \textbf{DAVE} \\
%     \midrule
%     ViT-B/16
%       & $0.461 \pm 0.159$
%       & $\textcolor{blue}{\mathbf{0.736 \pm 0.084}}$
%       & $0.509 \pm 0.123$
%       & $0.561 \pm 0.094$
%       & --
%       & $0.651 \pm 0.122$ \\
%     DeiT-B/16
%       & $0.431 \pm 0.114$
%       & $\textcolor{blue}{\mathbf{0.717 \pm 0.073}}$
%       & $0.478 \pm 0.104$
%       & --
%       & --
%       & $0.657 \pm 0.104$ \\
%     Bcos-ViT-B/16
%       & $0.560 \pm 0.145$
%       & --
%       & $0.583 \pm 0.117$
%       & --
%       & $0.806 \pm 0.085$
%       & $\textcolor{blue}{\mathbf{0.830 \pm 0.079}}$ \\
%     Bcos-ViT\_c-B/16
%       & $0.570 \pm 0.138$
%       & --
%       & $0.594 \pm 0.111$
%       & --
%       & $0.885 \pm 0.061$
%       & $\textcolor{blue}{\mathbf{0.901 \pm 0.064}}$ \\
%     DINO-ViT-B/16
%       & -- & -- & -- & -- & -- & -- \\
%     CLIP-ViT-B/16
%       & -- & -- & -- & -- & --  & --\\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}[t]
%   \centering
%   \caption{GridPG localisation scores on ImageNet, computed on $2{\times}2$ grids with cell size $224{\times}224$, comparing state-of-the-art explanation methods against DAVE (ours) for ViT-B/16-based architectures. Scores are reported as mean$\pm$std (over $n{=}500$ grid images). \sid{re-run this again, update DINO.}}
%   \label{tab:gridpg}

%   \scriptsize
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{0.92}

%   \resizebox{\columnwidth}{!}{%
%   \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{6}{c}{\textbf{GridPG} $\uparrow$} \\
%     \cmidrule(lr){2-7}
%     & \textbf{IxG}
%     & \makecell{\textbf{Attn}\\\textbf{LRP}}
%     & \textbf{IG}
%     & \makecell{\textbf{C-}\\\textbf{CAM}}
%     & \textbf{B-cos}
%     & \textbf{DAVE} \\
%     \midrule
%     ViT-B/16
%       & $\mstd{0.46}{0.16}$
%       & $\textcolor{blue}{\mathbf{\mstd{0.74}{0.08}}}$
%       & $\mstd{0.51}{0.12}$
%       & $\mstd{0.56}{0.09}$
%       & --
%       & $\mstd{0.65}{0.12}$ \\
%     DeiT-B/16
%       & $\mstd{0.43}{0.11}$
%       & $\textcolor{blue}{\mathbf{\mstd{0.72}{0.07}}}$
%       & $\mstd{0.48}{0.10}$
%       & --
%       & --
%       & $\mstd{0.66}{0.10}$ \\
%     Bcos-ViT-B/16
%       & $\mstd{0.56}{0.15}$
%       & --
%       & $\mstd{0.58}{0.12}$
%       & --
%       & $\mstd{0.81}{0.09}$
%       & $\textcolor{blue}{\mathbf{\mstd{0.83}{0.08}}}$ \\
%     Bcos-ViT\_c-B/16
%       & $\mstd{0.57}{0.14}$
%       & --
%       & $\mstd{0.59}{0.11}$
%       & --
%       & $\mstd{0.89}{0.06}$
%       & $\textcolor{blue}{\mathbf{\mstd{0.90}{0.06}}}$ \\
%     DINO-ViT-B/16 & -- & -- & -- & -- & -- & -- \\
%     CLIP-ViT-B/16 & -- & -- & -- & -- & -- & -- \\
%     \bottomrule
%   \end{tabular}%
%   }
% \end{table}

\begin{table}[t]
  \centering
  \caption{GridPG localisation scores on ImageNet, computed on $2{\times}2$ grids with cell size $224{\times}224$, comparing attribution methods across ViT-B/16-based architectures. Scores are reported as mean$\pm$std (std in subscript) and shown as percentages.}
  \label{tab:gridpg_transposed_pct}

  \scriptsize
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{0.92}

  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lccccc}
    \toprule
    \textbf{Method} & \textbf{ViT-B/16} & \textbf{DeiT-B/16} & \textbf{DeiT-III/16} & \textbf{Bcos-ViT-B/16} & \textbf{Bcos-ViT\_c-B/16} \\
    \midrule
    IxG
      & $\mstd{41.38}{12.36}\%$
      & $\mstd{46.88}{10.80}\%$
      & $\mstd{35.49}{12.92}\%$
      & $\mstd{56.10}{14.28}\%$
      & $\mstd{55.42}{14.56}\%$ \\
    AttnLRP
      & $\mstd{49.95}{11.31}\%$
      & $\mstd{52.39}{9.61}\%$
      & $\mstd{42.20}{8.70}\%$
      & --
      & -- \\
    IG
      & $\mstd{45.13}{9.73}\%$
      & $\mstd{50.48}{9.91}\%$
      & $\mstd{39.64}{12.32}\%$
      & $\mstd{58.27}{12.15}\%$
      & $\mstd{57.43}{11.86}\%$ \\
    C-CAM
      & $\mstd{55.03}{7.87}\%$
      & $\mstd{56.50}{7.82}\%$
      & --
      & --
      & -- \\
    B-cos
      & --
      & --
      & --
      & $\mstd{79.53}{8.19}\%$
      & $\mstd{87.61}{5.99}\%$ \\
    DAVE
      & $\mstd{64.52}{13.10}\%$
      & $\mstd{63.57}{10.14}\%$
      & $\mstd{65.83}{12.12}\%$
      & $\mstd{84.21}{9.31}\%$
      & $\mstd{88.45}{9.77}\%$ \\
    \bottomrule
  \end{tabular}%
  }
\end{table}

==> tables/pg_conventional.tex <==
\begin{table}[!t]
\centering
\scriptsize
\caption{\textbf{Localization on ViT/DeiT backbones.} GridPG (left) and Energy PG (right) on ImageNet-1k. $\Delta$ denotes the improvement of DAVE over the best competing method (higher is better).}

\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\columnwidth}{l *{3}{>{\centering\arraybackslash}X}  *{3}{>{\centering\arraybackslash}X}}
\toprule
& \multicolumn{3}{c}{\textbf{Grid PG} (\%)} & \multicolumn{3}{c}{\textbf{Energy PG}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Method & ViT-B & DeiT-B & \mbox{DeiT-III-B} & ViT-B & DeiT-B & \mbox{DeiT-III-B} \\
\midrule
I$\times$G         & 32.67 & 30.25 & 30.01 & 55.33 & 62.72 & 67.32 \\
IntGrad          & 39.86 & 36.11 & 31.68 & 58.51 & 64.22 & 68.12 \\
S-Grad  & 34.27 & 30.18 & 31.48 & 56.02 & 60.78 & 68.10 \\
LeGrad      & 47.71 & 42.58 & 34.62 & 80.06 & 77.83 & 77.54 \\
A-LRP     & 58.40 & 54.63 & 53.84 & 60.75 & 68.16 & 77.65 \\
C-LRP  & 54.98 & 55.47 & 52.27 & \textbf{80.82} & 79.62 & 81.94 \\

%\rowcolor{lightblue}
\rowcolor{davemauve!25}
DAVE (ours)        & \textbf{60.19} & \textbf{63.52} & \textbf{65.76} & 78.60 & \textbf{82.23} & \textbf{82.43} \\
\midrule
$\Delta$ 
& \textbf{\inc{+1.79}} & \textbf{\inc{+8.05}} & \textbf{\inc{+11.92}}
& \textcolor{red}{-2.22} &\textbf{ \inc{+2.61}} & \textbf{\inc{+0.49}} \\
\bottomrule
\end{tabularx}
%\vspace{-2mm}
%\caption{\textbf{Localization scores} (\%) on ViT/DeiT. Left: Grid PG. Right: Energy PG.}
\label{tab:pg_vit_deit_pct}
\end{table}


==> tables/pg_merged.tex <==
\begin{table*}[!t]
  \centering
  \scriptsize

  \begin{subtable}[t]{0.49\textwidth}
    \centering
    \setlength{\tabcolsep}{2.5pt}
    \renewcommand{\arraystretch}{1.12}
    \begin{tabularx}{\linewidth}{l *{3}{>{\centering\arraybackslash}X}  *{3}{>{\centering\arraybackslash}X}}
      \toprule
      & \multicolumn{3}{c}{\textbf{Grid PG} (\%)} & \multicolumn{3}{c}{\textbf{Energy PG}} \\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      Method & ViT-B & DeiT-B & \mbox{DeiT-III-B} & ViT-B & DeiT-B & \mbox{DeiT-III-B} \\
      \midrule
      I$\times$G         & 32.67 & 30.25 & 30.01 & 55.33 & 62.72 & 67.32 \\
      IntGrad            & 39.86 & 36.11 & 31.68 & 58.51 & 64.22 & 68.12 \\
      S-Grad             & 34.27 & 30.18 & 31.48 & 56.02 & 60.78 & 68.10 \\
      LeGrad             & 47.71 & 42.58 & 34.62 & 80.06 & 77.83 & 77.54 \\
      A-LRP              & 58.40 & 54.63 & 53.84 & 60.75 & 68.16 & 77.65 \\
      C-LRP              & 54.98 & 55.47 & 52.27 & \textbf{80.82} & 79.62 & 81.94 \\
      \rowcolor{davemauve!25}
      DAVE (ours)        & \textbf{60.19} & \textbf{63.52} & \textbf{65.76} & 78.60 & \textbf{82.23} & \textbf{82.43} \\
      \midrule
      $\Delta$
      & \textbf{\inc{+1.79}} & \textbf{\inc{+8.05}} & \textbf{\inc{+11.92}}
      & \textcolor{red}{-2.22} & \textbf{\inc{+2.61}} & \textbf{\inc{+0.49}} \\
      \bottomrule
    \end{tabularx}
    \caption{ViT/DeiT models.}
    \label{tab:pg_vit_deit_pct_sub}
  \end{subtable}\hfill
  \begin{subtable}[t]{0.49\textwidth}
    \centering
    \setlength{\tabcolsep}{3pt}
    \renewcommand{\arraystretch}{1.12}
    \begin{tabularx}{\linewidth}{l *{2}{>{\centering\arraybackslash}X}  *{2}{>{\centering\arraybackslash}X}}
      \toprule
      & \multicolumn{2}{c}{\textbf{Grid PG} (\%)} & \multicolumn{2}{c}{\textbf{Energy PG}} \\
      \cmidrule(lr){2-3}\cmidrule(lr){4-5}
      Method & B-cos-ViT & B-cos-ViT-C & B-cos-ViT & B-cos-ViT-C \\
      \midrule
      I$\times$G     & 55.71 & 55.38 & 65.29 & 66.72 \\
      IntGrad        & 57.98 & 57.68 & 65.33 & 67.75 \\
      S-Grad         & 60.27 & 61.30 & 68.16 & 69.59 \\
      \bcos          & 79.67 & 87.66 & 69.41 & 75.61 \\
      \rowcolor{davemauve!25}
      DAVE (ours)    & \textbf{84.00} & \textbf{88.43} & \textbf{78.55} & \textbf{79.63} \\
      \midrule
      $\Delta$       & \textbf{\inc{+4.33}} & \textbf{\inc{+0.77}} & \textbf{\inc{+9.14}} & \textbf{\inc{+4.02}} \\
      \bottomrule
    \end{tabularx}
    \caption{\bcos models.}
    \label{tab:pg_bcos_pct_sub}
  \end{subtable}

  \caption{\textbf{Localization scores} (\%) on (a) ViT/DeiT and (b) \bcos models. Left block: Grid PG. Right block: Energy PG.}
  \label{tab:pg_side_by_side}
\end{table*}

